Aero-engines Anomaly Detection using an Unsupervised Fisher Autoencoder

Reliable aero-engine anomaly detection is crucial for ensuring aircraft safety and operational efficiency. This research explores the application of the Fisher autoencoder as an unsupervised deep learning method for detecting anomalies in aero-engine multivariate sensor data, using a Gaussian mixture as the prior distribution of the latent space. The proposed method aims to minimize the Fisher divergence between the true and the modeled data distribution in order to train an autoencoder that can capture the normal patterns of aero-engine behavior. The Fisher divergence is robust to model uncertainty, meaning it can handle noisy or incomplete data. The Fisher autoencoder also has well-defined latent space regions, which makes it more generalizable and regularized for various types of aero-engines as well as facilitates diagnostic purposes. The proposed approach improves the accuracy of anomaly detection and reduces false alarms. Simulations using the CMAPSS dataset demonstrate the model's efficacy in achieving timely anomaly detection, even in the case of an unbalanced dataset.

==> anomalypaper.tex <==
@inproceedings{sowers2008application,
  title={Application of the systematic sensor selection strategy for turbofan engine diagnostics},
  author={Sowers, T Shane and Kopasakis, George and Simon, Donald L},
  booktitle={Turbo Expo: Power for Land, Sea, and Air},
  volume={43123},
  pages={135--143},
  year={2008}
}
